DeltaCam: Differential Intrinsic Camera Modeling for Video Generation

Incorporating camera intrinsics into video generation models offers a principled way to control not only scene dynamics but also the imaging process that governs visual appearance. Prior work has primarily focused on extrinsic control, such as camera pose and motion, while treating intrinsic camera parameters as implicit or fixed. A key bottleneck is the lack of large-scale video datasets with accurate and diverse temporally varying camera metadata, which makes learning absolute camera parameterizations difficult. As a result, current models struggle to incorporate photographic camera behavior, including depth-of-field transitions, exposure variations, lens distortions, and color processing, in a controllable and temporally consistent manner. We introduce DeltaCam, a video diffusion framework that models camera behavior through $\Delta$-parameterized neural camera adaptors, operating on relative changes in camera motion and intrinsics instead of absolute states. By learning this differential formulation from synthetic video data, we mitigate reliance on precise real-world camera labels and enable smooth, consistent control over imaging factors such as focal length, aperture, ISO, color temperature, and lens distortion. We extend this framework to real-world footage through two mechanisms: finetuning the controls on real image-metadata pairs for precise shot matching, and extracting disentangled embeddings for implicit video-to-video style transfer without requiring explicit camera parameters. By effectively separating scene content from intrinsic imaging behavior, DeltaCam enables camera-consistent video generation and editing operations that are difficult to achieve with existing models. Ultimately, our results establish a practical and scalable approach for bridging synthetic control and real-world photographic emulation.

==> acmart-support.tex <==
\clearpage
\pagenumbering{roman}
\input{content/supplement}


==> conf/packages.tex <==
%%% Language %%%%
\RequirePackage[english]{babel}                  % Hyphenation and date format
\RequirePackage{xspace}                          % Abbreviation spacing
\RequirePackage{xpunctuate}                      % Abbreviation spacing

%%% Tex-scripting %%%
\RequirePackage{ifthen}                          % If-then-else latex logic
\RequirePackage{soul}                            % Underlining and Strike-through
\RequirePackage{xargs}                           % For \newcommandx

%%% Color %%%
\RequirePackage{color}                           % Draft annotation coloring
\RequirePackage[dvipsnames]{xcolor} 

%%% Math-mode %%%
\RequirePackage{amsmath}                         % Math equations
\RequirePackage{bm}                              % Math bold symbols

\usepackage{adjustbox}
\usepackage{enumitem}
% \usepackage{todonotes}

\usepackage{multirow}
\usepackage[table]{xcolor}
\usepackage{graphicx}

% \usepackage[utf8]{inputenc}
\usepackage{multirow}
\usepackage{geometry}
\usepackage{subcaption}
 % \usepackage{algorithm}
 % \usepackage{algpseudocode}

 \usepackage{listings}
  \lstdefinestyle{pseudocode}{
    basicstyle=\footnotesize\ttfamily,
    commentstyle=\color{gray}\itshape,
    mathescape=true,
    escapeinside={(*}{*)},
    columns=flexible,
    keepspaces=true,
    morecomment=[l]{\#},
    frame=single,
    framesep=4pt,
    xleftmargin=6pt,
    xrightmargin=6pt,
  }



%%% Cross-referencing %%%
\RequirePackage[toc,page,titletoc]{appendix}     % Appendix section
\RequirePackage[capitalize,nameinlink]{cleveref} % Easy to use cross-referencing
\crefname{supp}{Supplement}{Supplements}     % Supplement section name setting

%%% Figures %%%
\RequirePackage{caption}                         % Figure captions
% \RequirePackage{subfig}                          % Nested figures

\usepackage{booktabs} % For formal tables
\usepackage{tabularx}
\usepackage{ragged2e}
\renewcommand\tabularxcolumn[1]{>{\Centering}m{#1}}

\usepackage{xcolor}
\newcommand\todo[1]{\textcolor{red}{#1}}

\usepackage{svg}
\usepackage{colortbl}
% tables
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\usepackage{makecell}












%%% Package options compaction %%%

% --- Compaction (safe with acmart + subfig) ---
\usepackage{microtype}

% Display math
\setlength{\abovedisplayskip}{3pt plus 1pt minus 1pt}
\setlength{\belowdisplayskip}{3pt plus 1pt minus 1pt}
\setlength{\abovedisplayshortskip}{0pt plus 1pt}
\setlength{\belowdisplayshortskip}{2pt plus 1pt minus 1pt}
\setlength{\jot}{2pt}

% Captions (acmart-safe: use captionsetup, not package options)
\captionsetup{font=small,labelfont=bf,skip=2pt,belowskip=2pt}
\setlength{\abovecaptionskip}{2pt}
\setlength{\belowcaptionskip}{2pt}
\setlength{\textfloatsep}{8pt plus 2pt minus 2pt}  % was 6pt

% Floats: separation
% \setlength{\textfloatsep}{6pt plus 2pt minus 2pt}
\setlength{\floatsep}{6pt plus 2pt minus 2pt}
% \setlength{\floatsep}{10pt plus 2pt minus 2pt}
\setlength{\intextsep}{6pt plus 2pt minus 2pt}
\setlength{\dbltextfloatsep}{6pt plus 2pt minus 2pt}
\setlength{\dblfloatsep}{6pt plus 2pt minus 2pt}
% \setlength{\dblfloatsep}{10pt plus 2pt minus 2pt}
% \setlength{\abovecaptionskip}{2pt}
% \setlength{\belowcaptionskip}{0pt}

% Floats: placement (lets LaTeX fill pages instead of pushing floats to the end)
\renewcommand{\topfraction}{0.95}
\renewcommand{\bottomfraction}{0.95}
\renewcommand{\textfraction}{0.05}
% \renewcommand{\floatpagefraction}{0.85}
\renewcommand{\dbltopfraction}{0.95}
% \renewcommand{\dblfloatpagefraction}{0.85}
\renewcommand{\floatpagefraction}{0.7}     % was 0.85 in my earlier suggestion
\renewcommand{\dblfloatpagefraction}{0.7}
\setcounter{topnumber}{3}
\setcounter{bottomnumber}{3}
\setcounter{totalnumber}{5}
\setcounter{dbltopnumber}{3}

% Lists (you already have enumitem)
\setlist{nosep,leftmargin=*}

% Line breaking
\emergencystretch=3em

\makeatletter
\setlength{\@fptop}{0pt}
\setlength{\@fpsep}{8pt plus 1pt}
\setlength{\@fpbot}{0pt plus 1fil}
\makeatother

==> content/figures/applications.tex <==

\begin{figure}[t]
    \includegraphics[width=\columnwidth]{assets/applications.pdf}
    \caption{\textit{Applications}. We show reversal of already existing effect in the source video. However, some effects such as temperature mildly \textit{overshoot} or show ``effect leaking" in the presence of existing effects in the input video.}
    \label{fig:applications}
    % \vspace{-0.5cm}
\end{figure}

==> content/figures/archi_evolution.tex <==

\begin{figure}[t]
    \includegraphics[width=\columnwidth]{assets/archi_evolution.pdf}
    \caption{\textit{Camera conditioning module architecture evolution}. }
    \label{fig:ccm_evolution}
    % \vspace{-0.5cm}
\end{figure}

==> content/figures/cam_data_adaptation.tex <==

\begin{figure}[t]
    \includegraphics[width=\columnwidth]{assets/camera_dataset_adaptation.pdf}
    \caption{\textit{Camera EXIF Data Video Adaptation}. }
    \label{fig:cam_adapt}
    % \vspace{-0.5cm}
\end{figure}

==> content/figures/dataset_preview.tex <==

\begin{figure}[t]
    \includegraphics[width=\columnwidth]{assets/dataset_preview.pdf}
    \caption{\textit{Dataset Composition}. }
    \label{fig:dataset_composition}
    % \vspace{-0.5cm}
\end{figure}

==> content/figures/demo.tex <==

\begin{figure}[t]
    \includegraphics[width=\columnwidth]{assets/demo.png}
    \caption{\textit{Our live demo can be viewed in the browser}. }
    \label{fig:demo}
    % \vspace{-0.5cm}
\end{figure}

==> content/figures/fidelity.tex <==

\begin{figure}[t]
    \includegraphics[width=\columnwidth]{assets/fidelity_ablations.pdf}
    \caption{\textit{Ablations: Effect fidelity}. }
    \label{fig:fidelity}
    % \vspace{-0.5cm}
\end{figure}

==> content/figures/latent_disentanglement.tex <==

\begin{figure}[t]
    \includegraphics[width=\columnwidth]{assets/layer_tsne.png}
    \caption{\textit{Ablations: CCM enforces latent disentanglement}. }
    \label{fig:latent_disent}
    % \vspace{-0.5cm}
\end{figure}

==> content/figures/loss.tex <==

\begin{figure}[t]
    \includegraphics[width=\columnwidth]{assets/training_curve_base.png}
    \caption{\textit{Training loss trajectory}. Combined denoising loss across the three training stages. Stage 1 (base camera model, 60K iters) shows the largest absolute decrease as the CCM aligns with the VDM latent space; Stages 2 (style adaptation, 15K iters) and 3 (EXIF matching, 6K iters) train only lightweight adaptors and converge quickly.}
    \label{fig:loss}
    % \vspace{-0.5cm}
\end{figure}

==> content/figures/recammaster.tex <==

\begin{figure}[t]
    \includegraphics[width=\columnwidth]{assets/zoom_recammaster.pdf}
    \caption{\textit{Comparison with ReCamMaster for focal length}. }
    \label{fig:focal}
    % \vspace{-0.5cm}
\end{figure}

==> content/figures/remain_comp.tex <==

\begin{figure}[t]
    \includegraphics[width=\columnwidth]{assets/fisheye_temperature.pdf}
    \caption{\textit{Comparison on lens distortion and color temperature}. }
    \label{fig:remain_comp}
    % \vspace{-0.5cm}
\end{figure}

==> content/figures/style_traj.tex <==

\begin{figure}[t]
    \includegraphics[width=\columnwidth]{assets/style_traj.pdf}
    \caption{\textit{Extracted Style Trajectories}. We show extracted style trajectories for camera parameters such as aperture for Bokeh and color temperature value. We show 3 samples per effect.}
    \label{fig:style_extraction_traj}
    % \vspace{-0.5cm}
\end{figure}

==> content/figures/supp_algo.tex <==
% \begin{figure*}[t]
%     \centering
%     \begin{minipage}[t]{0.47\textwidth}
%       \begin{lstlisting}[style=pseudocode]
%   def style_extract(X: (B, T, 3, H, W), concepts: List[str]):

%       # per-frame backbone (frozen c-RADIO v4 ViT-H)
%       summary, patches = cRADIO(X)           # (B,T,1280), (B,T,N,1280)
%       pooled = GaussianPool(patches, $\sigma$=0.3)  # uniform + radial + centre
%       H = Linear([summary; pooled])          # (B, T, 1280)

%       # shared temporal encoder
%       H = TransformerEncoder(H + SinPE,      # 4 layers, 8 heads,
%                              d=1280)         # feedforward = 4d

%       # content branch  ->  scene-identity vector
%       z_c = MLP(CrossAttn(q_learned, H))    # (B, 256),  depths 1280->2560->256

%       # style branch  ->  per-frame embeddings
%       Z_s = TransformerEncoder(H + SinPE,   # 4 layers, 8 heads
%                                d=1280)
%       Z_s = MLP(Z_s)                        # (B, T, 256),  1280->256

%       # per-concept trajectory heads
%       trajs = {}
%       for c in concepts:
%           trajs[c] = Linear(GELU(Linear(Z_s,  # 256 -> 128
%                                  128)), 1)    # 128 -> 1,  z-scored
%       return z_c, Z_s, trajs
%       \end{lstlisting}
%       \captionof{lstlisting}{Style extraction forward pass (one model per effect).}
%       \label{alg:style}
%     \end{minipage}    
%     \hfill
%     \begin{minipage}[t]{0.47\textwidth}
%       \begin{lstlisting}[style=pseudocode]
%   def recam_inference(X_src: (B,T,3,H,W), $\tau$: Dict[effect, (T,)],
%                       prompt: str, N: int = 50):

%       # --- proxy stream extraction (frozen) ---
%       D = DepthEstimator(X_src)           # (B, T, 1, H, W)
%       F = OpticalFlow(X_src)              # (B, T, 2, H, W)
%       P = PerspectiveField(X_src)         # (B, T, 4, H, W)

%       # --- VAE encoding ---
%       z_src   = VAE.encode(X_src)         # (B, 16, T', H', W')
%       z_depth = VAE.encode(D)             # (B, 16, T', H', W')
%       z_flow  = VAE.encode_multichan(F)   # (B, 32, T', H', W')
%       z_pf    = VAE.encode_multichan(P)   # (B, 64, T', H', W')

%       # --- camera control module (CCM) ---
%       x2d = [z_depth, z_flow, z_pf, z_src]
%       x1d = build_x1d($\tau$)                   # (B, 6, T', 8)
%       x1d_norm = [x1d_enc[j](x1d[:,j]) for j in effects]
%       acc = $\sum_{k,j}$ FiLM(InputProj(x2d[k]), x1d_norm[j])
%       for stage in [0, 1, 2]:
%           acc = CausalTemporalSelfAttn(StageProj(acc))
%       cam_emb1 = [OutProj[b](acc) for b in DiT.blocks]

%       # --- diffusion denoising loop ---
%       z = randn_like(z_src)
%       for t in FlowMatchScheduler.timesteps(N):
%           z_in = concat([z, z_src], dim=T)
%           x = PatchEmbed(z_in);  e = patchify1(cam_emb1)
%           for b, block in enumerate(DiT.blocks):
%               $\tilde{x}$ = AdaLN(x, t)
%               x1 = SA(    $\tilde{x}$ + CamEnc(e_scalar))
%               x2 = SA_eff($\tilde{x}$ + e[b])
%               x = x + $g_\text{msa}$ * 0.5*(P1(x1) + P2(x2))
%               x = x + CrossAttn(x, context) + $g_\text{mlp}$*FFN(AdaLN(x,t))
%           z = scheduler.step(Head(x), t, z)

%       return VAE.decode(z)                 # (B, T, 3, H, W)
%       \end{lstlisting}
%       \captionof{lstlisting}{Camera-conditioned VDM inference forward pass.}
%       \label{alg:inference}
%     \end{minipage}
%   \end{figure*}

\begin{figure*}[t]
    \centering
    \begin{minipage}[t]{0.47\textwidth}
      \begin{lstlisting}[style=pseudocode]
  def vdm_inference(X_src: (B,T,3,H,W), $\tau$: Dict[effect, (T,)],
                    prompt: str, N: int = 50):
  
      # --- proxy stream extraction (frozen) ---
      D = DepthEstimator(X_src)           # (B, T, 1, H, W)
      F = OpticalFlow(X_src)              # (B, T, 2, H, W)
      P = PerspectiveField(X_src)         # (B, T, 4, H, W)
  
      # --- VAE encoding ---
      z_src   = VAE.encode(X_src)         # (B, 16, T', H', W')
      z_depth = VAE.encode(D)             # (B, 16, T', H', W')
      z_flow  = VAE.encode_multichan(F)   # (B, 32, T', H', W')
      z_pf    = VAE.encode_multichan(P)   # (B, 64, T', H', W')

      # --- camera control module (CCM) ---
      x2d = [z_depth, z_flow, z_pf, z_src]
      x1d = build_x1d($\tau$)                   # (B, 6, T', 8)
      x1d_norm = [x1d_enc[j](x1d[:,j]) for j in effects]
      acc = $\sum_{k,j}$ FiLM(InputProj(x2d[k]), x1d_norm[j])
      for stage in [0, 1, 2]:
          acc = CausalTemporalSelfAttn(StageProj(acc))
      cam_emb1 = [OutProj[b](acc) for b in DiT.blocks]
  
      # --- diffusion denoising loop ---
      z = randn_like(z_src)
      for t in FlowMatchScheduler.timesteps(N):
          z_in = concat([z, z_src], dim=T)
          x = PatchEmbed(z_in);  e = patchify1(cam_emb1)
          for b, block in enumerate(DiT.blocks):
              $\tilde{x}$ = AdaLN(x, t)
              x1 = SA(    $\tilde{x}$ + CamEnc(e_scalar))
              x2 = SA_eff($\tilde{x}$ + e[b])
              x = x + $g_\text{msa}$ * 0.5*(P1(x1) + P2(x2))
              x = x + CrossAttn(x, context) + $g_\text{mlp}$*FFN(AdaLN(x,t))
          z = scheduler.step(Head(x), t, z)
  
      return VAE.decode(z)                 # (B, T, 3, H, W)
      \end{lstlisting}
      \captionof{lstlisting}{Camera-conditioned VDM inference forward pass.}
      \label{alg:inference}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.52\textwidth}
      \begin{lstlisting}[style=pseudocode]
  def style_extract(X: (B, T, 3, H, W), concepts: List[str]):

      # per-frame backbone (frozen c-RADIO v4 ViT-H)
      summary, patches = cRADIO(X)           # (B,T,1280), (B,T,N,1280)
      pooled = GaussianPool(patches, $\sigma$=0.3)  # uniform + radial + centre
      H = Linear([summary; pooled])          # (B, T, 1280)
  
      # shared temporal encoder
      H = TransformerEncoder(H + SinPE,      # 4 layers, 8 heads,
                             d=1280)         # feedforward = 4d

      # content branch  ->  scene-identity vector
      z_c = MLP(CrossAttn(q_learned, H))    # (B, 256),
                                            #  depths 1280->2560->256

      # style branch  ->  per-frame embeddings
      Z_s = TransformerEncoder(H + SinPE,   # 4 layers, 8 heads
                               d=1280)
      Z_s = MLP(Z_s)                        # (B, T, 256),  1280->256
  
      # per-concept trajectory heads
      trajs = {}
      for c in concepts:
          trajs[c] = Linear(GELU(Linear(Z_s,  # 256 -> 128
                                 128)), 1)    # 128 -> 1,  z-scored
      return z_c, Z_s, trajs
      \end{lstlisting}
      \captionof{lstlisting}{Style extraction forward pass (one model per pass).}
      \label{alg:style}
    \end{minipage}
  \end{figure*}

  


% \begin{figure}[t]
%   \begin{lstlisting}[style=pseudocode,
%     caption={Style extraction forward pass (one model per effect).},
%     label={alg:forward}]
%   def style_extract(X: (B, T, 3, H, W), concepts: List[str]):

%       # per-frame backbone (frozen c-RADIO v4 ViT-H)
%       summary, patches = cRADIO(X)           # (B,T,1280), (B,T,N,1280)
%       pooled = GaussianPool(patches, $\sigma$=0.3)  # uniform + radial + centre
%       H = Linear([summary; pooled])          # (B, T, 1280)

%       # shared temporal encoder
%       H = TransformerEncoder(H + SinPE,      # 4 layers, 8 heads,
%                              d=1280)         # feedforward = 4d

%       # content branch  ->  scene-identity vector
%       z_c = MLP(CrossAttn(q_learned, H))    # (B, 256),  depths 1280->2560->256

%       # style branch  ->  per-frame embeddings
%       Z_s = TransformerEncoder(H + SinPE,   # 4 layers, 8 heads
%                                d=1280)
%       Z_s = MLP(Z_s)                        # (B, T, 256),  1280->256

%       # per-concept trajectory heads
%       trajs = {}
%       for c in concepts:
%           trajs[c] = Linear(GELU(Linear(Z_s,  # 256 -> 128
%                                  128)), 1)    # 128 -> 1,  z-scored
%       return z_c, Z_s, trajs
%   \end{lstlisting}
%   \end{figure}


==> content/tables/abla_effect_stream.tex <==
% \begin{table}[h]
%   \centering
%   \caption{%
%     Stream-zeroing ablation. Each column reports the PSNR change (dB)
%     relative to the full model when the indicated 2-D proxy stream is
%     zeroed: depth, optical flow, perspective field, source video, or
%     all four simultaneously (\textbf{no\_2d}).
%     Full-model PSNR is listed for reference.
%   }
%   \label{tab:stream_ablation}
%   \setlength{\tabcolsep}{6pt}
%   \begin{tabular}{lc ccccc}
%   \toprule
%    & & \multicolumn{5}{c}{$\Delta$PSNR (dB) vs.\ Full} \\
%   \cmidrule(lr){3-7}
%   Effect & Full & no\_depth & no\_flow & no\_pf & no\_src & no\_2d \\
%   \midrule
%   Exposure     & 23.83 & $-$0.08 & $-$0.11 & $-$0.12 & $-$0.08 & $-$0.27 \\
%   Shutter      & 27.84 & $-$0.13 & $-$0.08 & $+$0.07 & $+$0.12 & $-$0.02 \\
%   Zooming      & 22.82 & $+$0.10 & $+$0.04 & $+$0.02 & $+$0.02 & $+$0.05 \\
%   Temperature  & 23.22 & $-$0.02 & $+$0.12 & $+$0.05 & $-$0.08 & $-$0.01 \\
%   Bokeh        & 20.75 & $-$0.61 & $+$0.06 & $-$0.03 & $+$0.03 & $-$0.52 \\
%   Fisheye      & 13.60 & $+$0.03 & $\phantom{+}$0.00 & $-$0.01 & $-$0.02 & $+$0.04 \\
%   \bottomrule
%   \end{tabular}
%   \end{table}

\begin{table}[h]
  \centering
  \caption{%
    Stream-zeroing ablation. Each column reports the PSNR change (dB)
    relative to the full model when the indicated 2-D proxy stream is
    zeroed. Cells are shaded white\,{\footnotesize(no dependence)} to
    red\,{\footnotesize(strong dependence)}, normalized to the maximum
    observed drop of $0.61$\,dB.
  }
  \label{tab:stream_ablation}
  \setlength{\tabcolsep}{6pt}
  \begin{tabular}{lc ccccc}
  \toprule
   & & \multicolumn{5}{c}{$\Delta$PSNR (dB) vs.\ Full} \\
  \cmidrule(lr){3-7}
  Effect & Full & no\_depth & no\_flow & no\_pf & no\_src & no\_2d \\
  \midrule
  Exposure      & 23.83 & \cellcolor[rgb]{1.00,0.87,0.87}$-$0.08 & \cellcolor[rgb]{1.00,0.82,0.82}$-$0.11 &
  \cellcolor[rgb]{1.00,0.80,0.80}$-$0.12 & \cellcolor[rgb]{1.00,0.87,0.87}$-$0.08 & \cellcolor[rgb]{1.00,0.56,0.56}$-$0.27 \\
  Shutter       & 27.84 & \cellcolor[rgb]{1.00,0.79,0.79}$-$0.13 & \cellcolor[rgb]{1.00,0.87,0.87}$-$0.08 & $+$0.07 & $+$0.12
   & $-$0.02 \\
  Zooming       & 22.82 & $+$0.10 & $+$0.04 & $+$0.02 & $+$0.02 & $+$0.05 \\
  Temperature   & 23.22 & $-$0.02 & $+$0.12 & $+$0.05 & \cellcolor[rgb]{1.00,0.87,0.87}$-$0.08 & $-$0.01 \\
  Bokeh         & 20.75 & \cellcolor[rgb]{1.00,0.00,0.00}$-$0.61 & $+$0.06 & $-$0.03 & $+$0.03 &
  \cellcolor[rgb]{1.00,0.15,0.15}$-$0.52 \\
  Fisheye       & 13.60 & $+$0.03 & $\phantom{+}$0.00 & $-$0.01 & $-$0.02 & $+$0.04 \\
  \bottomrule
  \end{tabular}
  \end{table}

==> content/tables/dataset_rdf.tex <==
\begin{table}[htbp]
    \centering
    \caption{\textbf{Real Data Finetuning} Comparison of various datasets by capture parameters.} 
    \label{tab:datasets_rdf}
    
    % Typography settings for a cleaner look
    \renewcommand{\arraystretch}{1.15} 
    \setlength{\tabcolsep}{4pt}
    \small 
    
    % Use adjustbox to ensure the table fits within the text width
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{@{} l c c c c c c c c c @{}}
        \toprule
        \textbf{Dataset} & \textbf{Size} & \textbf{$f$} & \textbf{$f/\#$} & \textbf{$\xi$} & \textbf{s} & \textbf{ISO} & \textbf{EV} & \textbf{K} & \textbf{CCM} \\
        \midrule
        BVI-Lowlight \cite{}   & -- & 600   & --   & --   & --  & -- & -- & -- & -- \\
        Zoom \cite{}           & -- & 585   & --   & --   & --  & -- & -- & -- & -- \\
        NeuralCam  \cite{}     & -- & 10k   & --   & --   & --  & -- & -- & -- & -- \\
        RealBokeh \cite{}      & -- & 23k   & --   & --   & --  & -- & -- & -- & -- \\
        BLB \cite{}      & -- & 23k   & --   & --   & --  & -- & -- & -- & -- \\
        WIFD \cite{}           & -- & 6k    & --   & --   & --  & -- & -- & -- & -- \\
        Real-HDRV \cite{}      & -- & --    & --   & --   & --  & -- & -- & -- & -- \\
        Funt et al. \cite{}        & -- & 15k   & --   & --   & --  & -- & -- & -- & -- \\
        ReDS \cite{}           & -- & 15k   & --   & --   & --  & -- & -- & -- & -- \\
        Adobe240 \cite{}            & -- & 15k   & --   & --   & --  & -- & -- & -- & -- \\
        CVRG \cite{}           & -- & 15k   & --   & --   & --  & -- & -- & -- & -- \\
        NTIRE360 \cite{}       & -- & 15k   & --   & --   & --  & -- & -- & -- & -- \\
        360SOD \cite{}         & -- & 15k   & --   & --   & --  & -- & -- & -- & -- \\
        \midrule
        \textbf{Total}  & & $\sim$\textbf{130k} & & & & & & & \\ 
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    
    \vspace{0.2cm}
    \footnotesize
    \textit{Note: ``--'' denotes data not available. Ranges are formatted as [min, max].}
\end{table}
